A Fast Randomized Algorithm for Massive Text Normalization

Many popular machine learning techniques in natural language processing and data mining rely heavily on high-quality text sources. However real-world text datasets contain a significant amount of spelling errors and improperly punctuated variants where the performance of these models would quickly deteriorate. Moreover, real-world, web-scale datasets contain hundreds of millions or even billions of lines of text, where the existing text cleaning tools are prohibitively expensive to execute over and may require an overhead to learn the corrections. In this paper, we present FLAN, a scalable randomized algorithm to clean and canonicalize massive text data. Our algorithm relies on the Jaccard similarity between words to suggest correction results. We efficiently handle the pairwise word-to-word comparisons via Locality Sensitive Hashing (LSH). We also propose a novel stabilization process to address the issue of hash collisions between dissimilar words, which is a consequence of the randomized nature of LSH and is exacerbated by the massive scale of real-world datasets. Compared with existing approaches, our method is more efficient, both asymptotically and in empirical evaluations, and does not rely on additional features, such as lexical/phonetic similarity or word embedding features. In addition, FLAN does not require any annotated data or supervised learning. We further theoretically show the robustness of our algorithm with upper bounds on the false positive and false negative rates of corrections. Our experimental results on real-world datasets demonstrate the efficiency and efficacy of FLAN.

==> tex/related-work.tex <==

\section{Related Work}
In the literature, the classic approaches for lexical normalization usually encompass a combination of spelling correction, stemming~\cite{4410417}, and regular expression filtering~\cite{10.1145/980972.980996}. More recent works have introduced unsupervised statistical models for text cleaning~\cite{contractor2010cleansing,aw2006phrase} or combining multiple heuristics to identify and normalize OOV words~\cite{han2011lexical}. one line of research have explored learning robust word representations through end-to-end neural networks as opposed to normalizing the data beforehand \cite{malykh-etal-2018-robust,doval2019towards} or directly fine-tuning the BERT models for lexical normalization task~\cite{muller2019enhancing}. Another group of works focus on directly learning over the subword level information, where character sequences or subword pairs are directly used for learning the representation without any correction steps~\cite{muller2019enhancing}.



%For computing several LSH signatures of the data vector, the last decade has witnessed a tremendous advance in reducing the amortized computational and memory requirements  For random projections based LSH, of which signed random projection is a special case, we can calculate $T$ LSH hashes of the data vector, with dimensions $d$, in time $O(d\log{d} + T)$, a significant improvement over $O(dT)$. This speedup is possible due to the theory of Fast-Johnson-Lindenstrauss transformation~\cite{DBLP:journals/siamcomp/AilonC09}. On the orthogonal side, even better speedup of $O(d + T)$ has been obtained with permutation-based LSH, such as minwise hashing, using ideas of densification~\cite{DBLP:conf/icml/Shrivastava17,DBLP:conf/icml/Shrivastava014,DBLP:conf/uai/Shrivastava014}. These drastic reductions in hashing time have been instrumental in making LSH based methods more appealing and practical.



% comments from WSDM 2021 reviewer 3
% The major speedup of the paper comes from a previous work on minwise hashing as the authors claim: “On the orthogonal side, even better speedup of O(d+T) has been obtained with permutation-based LSH, such as minwise hashing, using ideas of densification [26–28]. These drastic reductions in hashing time have been instrumental in making LSH based methods more appealing and practical.” Thus, the speedup of this method is not a novel contribution from the authors.

